Robotic Optimization of Powdered Beverages Leveraging Computer Vision and Bayesian Optimization

The growing demand for innovative research in the food industry is driving the adoption of robots in large-scale experimentation, as it offers increased precision, replicability, and efficiency in product manufacturing and evaluation. To this end, we introduce a robotic system designed to optimize food product quality, focusing on powdered cappuccino preparation as a case study. By leveraging optimization algorithms and computer vision, the robot explores the parameter space to identify the ideal conditions for producing a cappuccino with the best foam quality. The system also incorporates computer vision-driven feedback in a closed-loop control to further improve the beverage. Our findings demonstrate the effectiveness of robotic automation in achieving high repeatability and extensive parameter exploration, paving the way for more advanced and reliable food product development.

==> biblio.tex <==

\begin{thebibliography}{00}

\bibitem{beetz_robotic_2011}
M. Beetz, U. Klank, I. Kresse, A. Maldonado, L. Mösenlechner, D. Pangercic, T. Rühr, and M. Tenorth,
``Robotic roommates making pancakes,'' in \textit{2011 11th IEEE-RAS International Conference on Humanoid Robots}, Oct. 2011, pp. 529--536.

\bibitem{danno_cooking_2021}
D. Danno, S. Hauser, and F. Iida, ``Robotic cooking through pose extraction from human natural cooking using OpenPose,'' submitted to IAS-16 (16th International Conference on Intelligent Autonomous System), 2021.


\bibitem{arteaga1994systematic}
G. E. Arteaga, E. Li-Chan, M. C. Vazquez-Arteaga, and S. Nakai, 
``Systematic experimental designs for product formula optimization,'' \textit{Trends in Food Science \& Technology}, vol. 5, no. 8, pp. 243--254, 1994.

\bibitem{buttriss2013food}
J. L. Buttriss, 
``Food reformulation: the challenges to the food industry,'' \textit{Proceedings of the Nutrition Society}, vol. 72, no. 1, pp. 61--69, 2013.

\bibitem{ilic2023complexity}
S. Ilic and J. Hughes, 
``Complexity and Similarity Metrics for Unsupervised Identification of Programming Methods for Robot Cooking Tasks,'' in \textit{International Workshop on Human-Friendly Robotics}, 2023, pp. 61--73.

\bibitem{bollini_bakebot_nodate}
M. Bollini, J. Barry, and D. Rus, 
``Bakebot: Baking cookies with the pr2,'' in \textit{The PR2 workshop: results, challenges and lessons learned in advancing robots with a common platform, IROS}, 2011.

\bibitem{kang2022effects}
G. W. Kang, Z. Z. Piao, and J. Y. Ko, 
``Effects of water types and roasting points on consumer liking and emotional responses toward coffee,'' \textit{Food Quality and Preference}, vol. 101, p. 104631, 2022.

\bibitem{labbe2021impact}
D. Labbe, A. Rytz, A. Strube, and V. Leloup, 
``Impact of mug shape and beverage volume on instant coffee perception,'' \textit{Food Quality and Preference}, vol. 89, p. 104150, 2021.

\bibitem{huppertz2010foaming}
T. Huppertz, 
``Foaming properties of milk: A review of the influence of composition and processing,'' \textit{International Journal of Dairy Technology}, vol. 63, no. 4, pp. 477--488, 2010.

\bibitem{kulcu2018computer}
D. B. K{\"u}lc{\"u}, 
``Computer vision technology on food science,'' \textit{Karaelmas Fen ve M{\"u}hendislik Dergisi}, vol. 8, no. 1, pp. 403--409, 2018.

\bibitem{ma2016applications}
J. Ma, D.-W. Sun, J.-H. Qu, D. Liu, H. Pu, W.-H. Gao, and X.-A. Zeng, 
``Applications of computer vision for assessing quality of agri-food products: a review of recent research advances,'' \textit{Critical reviews in food science and nutrition}, vol. 56, no. 1, pp. 113--127, 2016.

\bibitem{duong2020review}
L. N. K. Duong, M. Al-Fadhli, S. Jagtap, F. Bader, W. Martindale, M. Swainson, and A. Paoli,
``A review of robotics and autonomous systems in the food industry: From the supply chains perspective,'' \textit{Trends in Food Science \& Technology}, vol. 106, pp. 355--364, 2020.

\bibitem{deotale2020foaming}
S. Deotale, S. Dutta, J. A. Moses, V. M. Balasubramaniam, and C. Anandharamakrishnan, 
``Foaming characteristics of beverages and its relevance to food processing,'' \textit{Food engineering reviews}, vol. 12, no. 2, pp. 229--250, 2020.

\bibitem{fang2007measurement}
Y. Fang, C. Selomulya, and X. D. Chen, 
``On measurement of food powder reconstitution properties,'' \textit{Drying technology}, vol. 26, no. 1, pp. 3--14, 2007.

\bibitem{kobayashi2015impact}
M. L. Kobayashi and M. de Toledo Benassi, 
``Impact of packaging characteristics on consumer purchase intention: Instant coffee in refill packs and glass jars,'' \textit{Journal of Sensory Studies}, vol. 30, no. 3, pp. 169--180, 2015.

\bibitem{shahriari2015taking}
B. Shahriari, K. Swersky, Z. Wang, R. P. Adams, and N. De Freitas,
``Taking the human out of the loop: A review of Bayesian optimization,'' \textit{Proceedings of the IEEE}, vol. 104, no. 1, pp. 148--175, 2015.


\bibitem{ha2015recent}
D. Ha, Q. Sun, K. Su, H. Wan, H. Li, N. Xu, F. Sun, L. Zhuang, N. Hu, and P. Wang,
``Recent achievements in electronic tongue and bioelectronic tongue as taste sensors,'' \textit{Sensors and Actuators B: Chemical}, vol. 207, pp. 1136--1146, 2015.




\bibitem{schuchmann2007product}
H. Schuchmann, 
``Product design for coffee based beverages,'' \textit{Product Design \& Engineering}, vol. 2, 2007.

\bibitem{juriaanse2006challenges}
A. C. Juriaanse, 
``Challenges ahead for food science,'' \textit{International journal of dairy technology}, vol. 59, no. 2, pp. 55--57, 2006.

\bibitem{tuorila2009sensory}
H. Tuorila and E. Monteleone, 
``Sensory food science in the changing society: Opportunities, needs, and challenges,'' \textit{Trends in Food Science \& Technology}, vol. 20, no. 2, pp. 54--62, 2009.

\bibitem{khan2018towards}
Z. H. Khan, A. Khalid, and J. Iqbal,
``Towards realizing robotic potential in future intelligent food manufacturing systems,'' \textit{Innovative food science \& emerging technologies}, vol. 48, pp. 11--24, 2018.



\bibitem{beet2011robotic}
M. Beetz, U. Klank, I. Kresse, A. Maldonado, L. Mösenlech-ner, D. Pangercic, T. Rühr, and M. Tenorth,
``Robotic roommates making pancakes,'' in \textit{2011 11th IEEE-RAS International Conference on Humanoid Robots}, Oct. 2011, pp. 529--536.


\bibitem{bollini2011bakebot}
M. Bollini, J. Barry, and D. Rus, 
``Bakebot: Baking cookies with the pr2,'' in \textit{The PR2 workshop: results, challenges and lessons learned in advancing robots with a common platform, IROS}, 2011.


\bibitem{satici2016coordinate}
A. Satici, F. Ruggiero, V. Lippiello, and B. Siciliano, 
``A Coordinate-Free Framework for Robotic Pizza Tossing and Catching,'' in \textit{2016 IEEE International Conference on Robotics and Automation (ICRA)}, May 2016, pp. 3932--3939.





\bibitem{junge_improving_2020}
K. Junge, J. Hughes, T. G. Thuruthel, and F. Iida, 
``Improving Robotic Cooking Using Batch Bayesian Optimization,'' \textit{IEEE Robotics and Automation Letters}, vol. 5, no. 2, pp. 760--765, 2020.

\bibitem{sochacki2021closed}
G. Sochacki, J. Hughes, F. Iida, and S. Hauser, 
``Closed-Loop Robotic Cooking of Scrambled Eggs with a Salinity-based ‘Taste’ Sensor,'' in \textit{International Conference on Intelligent Robots and Systems}, 2021.

\bibitem{sochacki2021compliant}
G. Sochacki, F. Iida, and J. Hughes, 
``Compliant Sensorized Testing Device to Provide a Model-Based Estimation of the Cooking Time of Vegetables,'' in \textit{16th International Conference On Intelligent Autonomous System}, 2021.

\bibitem{shweta2020foaming}
S. Deotale, S. Dutta, J. A. Moses, V. M. Balasubramaniam, and C. Anandharamakrishnan, 
``Foaming characteristics of beverages and its relevance to food processing,'' \textit{Food Engineering Reviews}, vol. 12, no. 2, pp. 229--250, 2020.

\bibitem{iqbal2017prospects}
J. Iqbal, Z. H. Khan, and A. Khalid, 
``Prospects of robotics in food industry,'' \textit{Food Science and Technology}, vol. 37, pp. 159--165, 2017.

\bibitem{scimeca2019nondestructive}
L. Scimeca, P. Maiolino, D. Cardin-Catalan, A. P. del Pobil, A. Morales, and F. Iida,
``Non-Destructive Robotic Assessment of Mango Ripeness via Multi-Point Soft Haptics,'' in \textit{2019 International Conference on Robotics and Automation (ICRA)}, 2019, pp. 1821--1826.

\bibitem{banga2003improving}
J. R. Banga, E. Balsa-Canto, C. G. Moles, and A. A. Alonso, 
``Improving food processing using modern optimization methods,'' \textit{Trends in Food Science \& Technology}, vol. 14, no. 4, pp. 131-144, 2003.


\bibitem{hendriks2020improvement}
K. Hendriks, 
``The improvement of objective milkfoam quality analysis through image processing and computer vision,'' Bachelor thesis, August 2020. [Online]. Available: \url{http://essay.utwente.nl/85547/}.
















\bibitem{nguyen2019bayesian}
V. Nguyen, "Bayesian Optimization for Accelerating Hyper-Parameter Tuning", \textit{2019 IEEE Second International Conference on Artificial Intelligence and Knowledge Engineering (AIKE)}, Sardinia, Italy, 2019, pp. 302-305, doi: 10.1109/AIKE.2019.00060.









\bibitem{saar2018modelfree}
K. Saar, F. Giardina, and F. Iida, 
``Model-Free Design Optimization of a Hopping Robot and Its Comparison With a Human Designer,'' \textit{IEEE Robotics and Automation Letters}, vol. PP, pp. 1-1, 2018.

\bibitem{Romachev2020flotation}
A. Romachev, V. Kuznetsov, E. Ivanov, and J. Benndorf, 
``Flotation froth feature analysis using computer vision technology,'' \textit{E3S Web of Conferences}, vol. 192, p. 02022, 2020.

\bibitem{Kawaharazuka2024continuous}
K. Kawaharazuka, N. Kanazawa, Y. Obinata, K. Okada, and M. Inaba,
``Continuous Object State Recognition for Cooking Robots Using Pre-Trained Vision-Language Models and Black-Box Optimization,'' \textit{IEEE Robotics and Automation Letters}, vol. 9, no. 5, pp. 4059-4066, 2024.

\bibitem{sakib2024from}
M. S. Sakib and Y. Sun, 
``From Cooking Recipes to Robot Task Trees – Improving Planning Correctness and Task Efficiency by Leveraging LLMs with a Knowledge Network,'' in \textit{2024 IEEE International Conference on Robotics and Automation (ICRA)}, 2024, pp. 12704-12711.

\bibitem{min12091126}
W. Zhang, D. Liu, C. Wang, R. Liu, D. Wang, L. Yu, and S. Wen, 
``An Improved Python-Based Image Processing Algorithm for Flotation Foam Analysis,'' \textit{Minerals}, vol. 12, no. 9, p. 1126, 2022.

\bibitem{Cimini2016}
A. Cimini, F. Pallottino, P. Menesatti, and M. Moresi, 
``A Low-Cost Image Analysis System to Upgrade the Rudin Beer Foam Head Retention Meter,'' \textit{Food and Bioprocess Technology}, vol. 9, no. 9, pp. 1587--1597, 2016.

\bibitem{GONZALEZVIEJO2016504}
C. G. Viejo, S. Fuentes, G. Li, R. Collmann, B. Condé, and D. Torrico,
``Development of a robotic pourer constructed with ubiquitous materials, open hardware and sensors to assess beer foam quality using computer vision and pattern recognition algorithms: RoboBEER,'' \textit{Food Research International}, vol. 89, pp. 504-513, 2016.

\bibitem{BARKER2002565}
G. S. Barker, B. Jefferson, and S. J. Judd, 
``The control of bubble size in carbonated beverages,'' \textit{Chemical Engineering Science}, vol. 57, no. 4, pp. 565-573, 2002.

\bibitem{ALDRICH2022107823}
C. Aldrich, E. Avelar, and X. Liu,
``Recent advances in flotation froth image analysis,'' \textit{Minerals Engineering}, vol. 188, p. 107823, 2022.

\bibitem{Viejo2019}
C. G. Viejo, D. D. Torrico, F. R. Dunshea, and S. Fuentes,
``Bubbles, Foam Formation, Stability and Consumer Perception of Carbonated Drinks: A Review of Current, New and Emerging Technologies for Rapid Assessment and Control,'' \textit{Foods}, vol. 8, no. 12, p. 596, 2019.

\bibitem{liu2022stirfry}
J.~Liu, Y.~Chen, Z.~Dong, S.~Wang, S.~Calinon, M.~Li, and F.~Chen, ``Robot cooking with stir-fry: Bimanual non-prehensile manipulation of semi-fluid objects,'' \emph{IEEE Robotics and Automation Letters}, vol.~7, no.~2, pp. 5159--5166, 2022, doi: 10.1109/LRA.2022.3153728.

\bibitem{eng4040143}
M.~Schmitz, F.~Menz, R.~Grunau, N.~Mandischer, M.~Hüsing, and B.~Corves, ``Robot cooking—Transferring observations into a planning language: An automated approach in the field of cooking,'' \textit{Eng}, vol.~4, no.~4, pp. 2514--2524, 2023. [Online]. Available: \url{https://www.mdpi.com/2673-4117/4/4/143}. doi: 10.3390/eng4040143.


\bibitem{Satici2022}
A.~C.~Satici, F.~Ruggiero, V.~Lippiello, and B.~Siciliano, ``A coordinate-free framework for robotic pizza tossing and catching,'' in \textit{Robot Dynamic Manipulation}, B.~Siciliano and F.~Ruggiero, Eds. Springer Tracts in Advanced Robotics, vol. 144, Springer, Cham, 2022. doi: 10.1007/978-3-030-93290-9\_8.


\bibitem{Zhao2015}
H.~Zhao, X.~Hao, A.~Wang, and C.~Li, ``Design and implementation of an intelligent cooking robot based on Internet of Things,'' in \emph{Proceedings of the 2015 Chinese Intelligent Automation Conference}, Z.~Deng and H.~Li, Eds., Lecture Notes in Electrical Engineering, vol. 338, Springer, Berlin, Heidelberg, 2015. doi: 10.1007/978-3-662-46466-3\_42.

\bibitem{watanabe2023treestructuredparzenestimatorunderstanding}
S.~Watanabe, ``Tree-Structured Parzen Estimator: Understanding Its Algorithm Components and Their Roles for Better Empirical Performance,'' 2023. [Online]. Available: \url{https://arxiv.org/abs/2304.11127}.


\end{thebibliography}

